Device Variability Analysis for Memristive Material Implication

Currently, memristor devices suffer from variability between devices and from cycle to cycle. In this work, we study the impact of device variations on memristive Material Implication (IMPLY). New constraints for different parameters and variables are analytically derived and compared to extensive simulation results, covering single gate and 1T1R crossbar structures. We show that a static analysis based on switching conditions is not sufficient for an overall assessment of robustness against device variability. Furthermore, we outline parameter ranges within which the IMPLY gate is predicted to produce correct output values. Our study shows that threshold voltage is the most critical parameter. This work helps scientists and engineers to understand the pitfalls of designing reliable IMPLY-based calculation units better and design them with more ease. Moreover, these analyses can be used to determine whether a certain memristor technology is suitable for implementation of IMPLY-based circuits and systems.

==> ArXiv_TNanoTech - Reliability Analysis of IMPLY Logic in ReRAM/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%						Acronyms							   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[acronym]{glossaries} % Acronyms
%\makeglossaries


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Health-care (alphabetic order):							   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{asd}{ASD}{Autism Spectrum Disorder}
\newacronym{cart}{CART}{Classification And Regression Tree}
\newacronym{dfa}{DFA}{Discriminant Function Analysis} 
\newacronym{ecg}{ECG}{Electrocardiography}
\newacronym{skin_eda}{EDA}{Electrodermal activity} 		
%In conflict with SoC definition
\newacronym{ews}{EWS}{Early Warning Score}
\newacronym{ga}{GA}{Genetic Algorithm}
\newacronym{hr}{HR}{Heart Rate}
\newacronym{ldf}{LDF}{Linear Discriminant Function}
\newacronym{rmsdd}{RMSDD}{Root-Mean Square of Successive Differences}
\newacronym{rsvm}{RSVM}{Reputation-driven Support Vector Machine }
\newacronym{saews}{SA-EWS}{Self-Aware Early Warning Score}
\newacronym{sam}{SAM}{Self-Assessment Manikin} 
\newacronym{selphys}{SelPhyS}{Self-aware cyber-Physical System}
\newacronym{sdnn}{SDNN}{Standard Deviation Normal-to-Normal-Intervals}
\newacronym{skt}{SKT}{Skin Temperature}
\newacronym{som}{SOM}{Self-Organizing Map}
\newacronym{whs}{WHS}{Wearable Health-care Systems}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Learning:													   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{ann}{ANN}{Artificial Neural Network}
\newacronym{bpn}{BPN}{Back-Propagation Neural Network}
\newacronym{bpnn}{BPNN}{back-propagation neural network}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{flop}{FLOP}{Floating Point Operation}
\newacronym{icnn}{ICNN}{Iterative Convolutional Neural Network}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym{nn}{NN}{Neural Network}
\newacronym{nb}{NB}{Naive Bayesian}
\newacronym{mcs}{MCS}{Multiple Classifier System}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{ucnn}{$\mu$CNN}{Micro CNN}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Memristor (alphabetic order):								   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{brs}{BRS}{Bipolar Resistive Switch-based logic}
\newacronym{cnf}{CNF}{Conjunctive Normal Form}
\newacronym{crs}{CRS}{Complementary Resistive Switch-based logic}
\newacronym{dnf}{DNF}{Disjunctive Normal Form}
\newacronym{ecm}{ECM}{Electrochemical Metallization}
\newacronym{fpm}{FPM}{Forward Polarized Memristor}
\newacronym{hfo}{$HfO_x$}{Hafnium Oxide}
\newacronym{hrs}{HRS}{High Resistance State}
\newacronym{imc}{IMC}{In-Memory Computation}
\newacronym{imply}{IMPLY}{Material Implication}
\newacronym{imp}{IMP}{In-Memory Processing}
\newacronym{lim}{LIM}{Logic in Memory}
\newacronym{lrs}{LRS}{Low Resistance State}
\newacronym{ltg}{LTG}{Logic Threshold Gate}
\newacronym{magic}{MAGIC}{Memristor-Aided Logic}
\newacronym{mecoins}{Me-Coin}{Memristor-based Computation In-memory}
\newacronym{nimp}{NIMP}{NOT IMPLY}
\newacronym{pc}{PC}{Phase Change}
\newacronym{pcm}{PCM}{Phase Change Memory}
\newacronym{pim}{PIM}{Processing in Memory}
\newacronym{reram}{ReRAM}{Resistive Random Access Memory}
\newacronym{rpm}{RPM}{Reversely Polarized Memristor}
\newacronym{stt}{STT}{Spin Transfer Torque}
\newacronym{tao}{$TaO_x$}{Tantalum Oxide}
\newacronym{tio}{$TiO_2$}{Titanium dioxide}
\newacronym{vc}{VC}{Valence Change}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Self-awareness (alphabetic order):						   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{aco}{ACO}{Autonomous Cooperating Object}
\newacronym{afdd}{AFDD}{Automated Fault Detection and Diagnostic}
\newacronym{ca}{CA}{Continuous Average}
\newacronym{cah}{CAH}{Context-Aware Health Monitoring}
\newacronym{cam}{CCAM}{Confidence-based Context-Aware condition Monitoring}
%\newacronym{cam}{C\textsuperscript{2}AM}{Confidence-based Context-Aware health Monitoring}
\newacronym[plural=DABs,longplural={Discrete Average Blocks}]{dab}{DAB}{Discrete Average Block}
\newacronym[plural=KPNs,longplural={Kahn Process Networks}]{kpn}{KPN}{Kahn Process Networks} 
\newacronym{mape-k}{MAPE-K}{Monitor-Analyze-Plan-Execute over a shared Knowledge}
\newacronym[plural=MoCs,longplural={Models of Computation}]{moc}{MoC}{Model of Computation}
\newacronym{oda}{ODA}{Observe-Decide-Act}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{rosa}{RoSA}{Research on Self-Awareness}
\newacronym{sa}{SA}{Self-Aware}
\newacronym{saness}{SA}{Self-Awareness}
\newacronym{sahm}{SAHM}{Self-Aware Health Monitoring}
\newacronym{samba}{SAMBA}{Self-Aware health Monitoring and Bio-inspired coordination for distributed Automation systems}
%\newacronym{sc}{SC}{Stability Controller}
\newacronym{sh}{SH}{State Handler}
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Systems (alphabetic order):								   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{cps}{CPS}{Cyber-Physical System}
\newacronym{cpps}{CPPS}{Cyber-Physical Production System}
\newacronym{dsr}{DSR}{Down-Sampling Rate}
\newacronym{dum}{DuM}{Device under Monitoring}
\newacronym{es}{ES}{Embedded System}
\newacronym{mes}{MES}{Manufacturing Execution System}
\newacronym{sos}{SoS}{System of Systems}
\newacronym{suo}{SuO}{System under Observation}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% System on Chip (alphabetic order):						   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{abi}{ABI}{Application Binary Interface}
\newacronym{adc}{ADC}{Analog-to-Digital Converter}
\newacronym{aes}{AES}{Advanced Encryption Standard}
\newacronym{alu}{ALU}{Arithmetic Logic Unit}
\newacronym{api}{API}{Application Programming Interface}
\newacronym{asic}{ASIC}{Application Specific Integrated Circuit}
\newacronym{asoc}{ASOC}{Autonomic System-on-Chip platform}
\newacronym{axi}{AXI}{Advanced eXtensible Interface Bus}
\newacronym{bram}{BRAM}{Block Random Access Memory}
\newacronym{cdt}{CDT}{C/C++ Development Tooling}
\newacronym{clb}{CLB}{Configuarable Logic Block}
\newacronym{cmos}{CMOS}{Complementary Metal-Oxide Semiconductor}
\newacronym{cp}{CP}{Clock Pulse}
\newacronym{cpi}{CPI}{Cycles Per Instruction}
\newacronym{cpu}{CPU}{Central Processing Unit} 
\newacronym{cpsoc}{CPSoC}{Cyber-Physical System-on-Chip}
\newacronym{cu}{CU}{Compute Unit}
\newacronym{cuda}{CUDA}{Compute Unified Device Architecture}
\newacronym{dac}{DAC}{Digital to Analog Converter}
\newacronym{ddr3}{DDR3}{Double Data Rate}
\newacronym{dff}{DFF}{Data Flip-Flop}
\newacronym{dll}{DLL}{Delay Locked Loop}
\newacronym{dmr}{DMR}{Dual Modular Redundancy}
\newacronym{dram}{DRAM}{Dynamic Random Access Memory}
\newacronym{dsd}{DSD}{Digital Synchronous Detection}
\newacronym{dsp}{DSP}{Digital Signal Processor}
\newacronym{dt}{DigiTime}{}
\newacronym{dvfs}{DVFS}{Dynamic Voltage and Frequency Scaling}
\newacronym{eda}{EDA}{Electronic Design Automation}
\newacronym{fdc}{FDC}{Frequency-to-Digital Converter}
\newacronym{fifo}{FIFO}{First In First Out}
\newacronym{fpga}{FPGA}{Field Programmable Gate Array}
\newacronym{gds}{GDS}{Global Data Share}
\newacronym{gnulgpl}{GNU LGPL}{GNU Lesser General Public Licence} 
\newacronym{gpgpu}{GPGPU}{General Purpose Graphics Processing Unit}
\newacronym{gpr}{GPR}{General Purpose Register}
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{gro}{GRO}{Gated Ring Oscillator}
\newacronym{io}{IO}{Input-Output}
\newacronym{hamsoc}{HAMSoC}{Hierarchical Agent Monitoring System-on-Chip}
\newacronym{hdl}{HDL}{Hardware Description Language}
\newacronym{hmp}{HMP}{Heterogeneous Multi-Processor}
\newacronym{ic}{IC}{Integrated Circuit}
\newacronym{icap}{ICAP}{Internal Configuration Access Port}
\newacronym[longplural={Intellectual Properties}]{ip}{IP}{Intellectual Property}
\newacronym{isa}{ISA}{Instruction Set Architecture}
\newacronym{lds}{LDS}{Local Data Share}
\newacronym{lru}{LRU}{Least Recently Used}
\newacronym{lsb}{LSB}{Least-Significant Bit}
\newacronym{lsu}{LSU}{Load Store Unit}
\newacronym{lut}{LUT}{Look Up Table}
\newacronym{mash}{MASH}{Multi-Stage Noise-Shaping}
\newacronym{mems}{MEMS}{Micro-Electro-Mechanical Systems}
\newacronym{miaow}{MIAOW}{Many-core Integrated Accelerator Of deepwater/Wisconsin}
\newacronym{mosfet}{MOSFET}{Metal Oxide Semiconductor Field Effect Transistor}
\newacronym{mpsoc}{MPSoC}{Multi-Processor System-on-Chip}
\newacronym{mshr}{MSHR}{Miss Status Holding/Handling Register}
\newacronym{noc}{NoC}{Network-on-Chip}
\newacronym{opencl}{OpenCL}{Open Computing Language}
\newacronym{ocn}{OCN}{On-Chip Network}
\newacronym{pcb}{PCB}{Printed Circuit Board}
\newacronym{pcie}{PCIe}{Peripheral Component Interconnect Express}
\newacronym{pl}{PL}{Programmable Logic}
\newacronym{pli}{PLI}{Verilog Programming Language Interface}
\newacronym{pll}{PLL}{Phase-Locked Loop}
\newacronym{ps}{PS}{Processing System}
\newacronym{pv}{PV}{Process Variation}
\newacronym{qoe}{QoE}{Quality of Experience}
\newacronym{qos}{QoS}{Quality of Service}
\newacronym{ram}{RAM}{Random Access Memory} 
\newacronym{risc}{RISC}{Reduced Instruction Set Computer}
\newacronym{riscv}{RISC-V}{Reduced Instruction Set Computing - V}
\newacronym{rtl}{RTL}{Register-Transfer Level}
\newacronym{sdk}{SDK}{Software Development Kit}
\newacronym{seec}{SEEC}{SElf-awarE Computing}
\newacronym{sgpr}{SGPR}{Scalar General Purpose Register}
\newacronym{si}{SI}{Southern Island}
\newacronym{simd}{SIMD}{Single Instruction Multiple Data}
\newacronym{simf}{SIMF}{Single Instruction Multiple Floating point}
\newacronym{sm}{SM}{Streaming Multiprocessor}
\newacronym{snr}{SNR}{Signal to Noise Ratio}
\newacronym[plural=SoCs,firstplural=Systems on Chip (SoCs)]{soc}{SoC}{System-on-Chip}
\newacronym{spared}{SPARED}{Self-aware PArtial Reconfiguration architecture for Edge Devices}
\newacronym{spice}{SPICE}{Simulation Program With Integrated Circuit Emphasis}
\newacronym{tad}{TAD}{Time \gls{adc}}
\newacronym[plural=TDCs,longplural={Time-to-Digital Converters}]{tdc}{TDC}{Time-to-Digital Converter}
\newacronym{tq}{TQ}{Time-Quantizer}
\newacronym{uart}{UART}{Universal Asynchronous Receiver/Transmitter}
\newacronym{vcdu}{VCDU}{Voltage Controlled Delay Unit}
\newacronym{vco}{VCO}{Voltage Controlled Oscillator}
\newacronym{vga}{VGA}{Video Graphics Array}
\newacronym{vhdl}{VHDL}{Very High Speed Integrated Circuit Hardware Description Language}
\newacronym{vlsi}{VLSI}{Very Large Scale Integration}
\newacronym{vgpr}{VGPR}{Vector General Purpose Register}
\newacronym{xilffs}{XILFFS}{Generic Fat File System Library}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%General (uncategorized):									   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newacronym{amd}{AMD}{Advanced Micro Devices}
\newacronym{beol}{BEOL}{Back End Of Line}
\newacronym{cad}{CAD}{Computer-Aided Design}
\newacronym{cas}{CAS}{Circuits and Systems}
\newacronym{eu}{EU}{European Union}
\newacronym{fdd}{FDD}{fault detection and diagnostic}
\newacronym{fefet}{FeFET}{Ferroelectric Field Effect Transistor}
\newacronym{feline}{FeLINe}{FeFET Logic IN mEmory}
\newacronym[plural=FOMs,longplural={Figures of Merit}]{fom}{FoM}{Figure of Merit}
\newacronym{hipeac}{HiPEAC}{High Performance and Embedded Architecture and Compilation}
\newacronym{hp}{HP}{Hewlett Packard}
\newacronym{hqp}{HQP}{Highly Qualified People}
\newacronym{hvac}{HVAC}{Heating, Ventilation and Air Conditioning}
\newacronym{ibm}{IBM}{International Business Machines corporation}
\newacronym{ict}{ICT}{Institute for Computer Technology}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{kcl}{KCL}{Kirchhoff's circuit laws}
\newacronym{nda}{NDA}{Non-Disclosure Agreement}
\newacronym{nvp}{NVP}{Non-Volatile Processor}
\newacronym{oecd}{OECD}{Organization for Economic Cooperation and Development}
\newacronym{rd}{R\&D}{Research and Development}
\newacronym{soa}{SoA}{State-of-the-Art}
\newacronym{tsmc}{TSMC}{Taiwan Semiconductor Manufacturing Company}
\newacronym{tvlsi}{TVLSI}{Transactions on Very Large Scale Integration}













==> ArXiv_TNanoTech - Reliability Analysis of IMPLY Logic in ReRAM/acronyms_local.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Local Acronyms (alphabetic order):						   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newacronym{acr}{ACR}{Acronym}

==> ArXiv_TNanoTech - Reliability Analysis of IMPLY Logic in ReRAM/setup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set up document by Nima Taherinejad (c)
% V1.0 Last Update: 11/June/2018
% TextA & TextB are independent and cannot be combined
% Therefore TextA & TextB are mainly used for alternative texts,
% that is if you want to use  
% EITHER the text in TextA OR the text in TextB. 
% For simple redactions, please use Rdi
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Usage of this file (copy-paste and toggle comments once):	   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %instructions for using setup.tex
% \def\mode{0}  %Document (appearance) Mode. part of setup: 
%    % 0: Nothing is redacted.
%    %0=proofread (to do note comments and color texts stay)
%    %1=draft watermark, (comments and colors are eliminated)
%    %2=confidential watermark, (comments and colors are eliminated) 
%    %3=final (comments and colors are eliminated,         confidential data is removed    \begin{conf} conf data \end{conf})

% \def\redactionmode{1} %redaction mode: 0=none, i=redaction level i (upto4)
%    % 1: (2Detailed) Too Much Details
%    % 2: (Uncritical) Information that is not very important but it could be there, space permitting
%    % 3: (2SaveSpace) Information that is rather relevant/important but could be deleted if short of space
%    % 4: (IfMustDelete) Information that is important but can be dropped in extreme cases of limited space
%    %\begin{RedactionName} TEXT \end{RedactionName}   for different redaction of Text (RedactionName is one of the 4 above, 2Detailed, Uncritical, etc.)
%	 % Please make sure that \begin and \end comment are not indented
%	 % moreover, there should be an enter after the command and no comment

% \def\alttextmode{1} %alternative text mode mode: 0=A&B, 1: A & not B, 2: not A & B, 3, Not A & Not B

% \include{setup}

% %acronyms bank
% \include{acronyms}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%General Packages (alphabetic order):						   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{adjustbox}              % For adjusting the box size (of tables)
\usepackage{amsmath,amssymb}
%\usepackage{algorithmic}
\usepackage[english]{babel}
\usepackage{cite}					% either cite or natbib
\usepackage[dvipsnames]{xcolor} % needs to be included before any TikZ package
\usepackage[oldvoltagedirection]{circuitikz}
\usetikzlibrary{patterns}
\usepackage[hidelinks]{hyperref} % needs to be included before cleveref
\usepackage{cleveref}
\usepackage{comment}  				% for confidential environment
%\usepackage{enumerate} 				% for alphanumerical enumerate  [(a)] [(i)]. Commented in favor of enumitem, that one seams more complete and has more support/features.
\let\labelindent\relax
\usepackage{enumitem}				% for no indentation in itemize and roman or alphanumerical enumerate
\usepackage[T1]{fontenc}
\usepackage{graphicx}
	\graphicspath{{./img/}}		% to set the figures path
%\usepackage[hidelinks]{hyperref} % ghost -> needs to be included before cleveref
\usepackage[utf8]{inputenc}
\usepackage{multirow}				% multirow for tables
%\usepackage{natbib}					% either cite or natbib
\usepackage{pgfplots}
\pgfplotsset{compat=1.16}
\usepackage{tabularx} 				% extra features for tabular environment
\usepackage{threeparttable}
%\usepackage{todonotes} 			% is already embedded! in document modes
\usepackage{subfigure}
\usepackage{soul} 					%for highlighting
\usepackage{xargs}    				% for newcommandx definitions % e.g. notes & colors
%\usepackage[]{xcolor}			% ghost --> needs to be included before TikZ



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%General Definitions										   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\plan}[1]{\todo[inline, linecolor=blue,backgroundcolor=blue!25,bordercolor=blue]{Plan: #1}}
\newcommand{\nimat}[1]{\todo[inline, linecolor=red,backgroundcolor=green!25,bordercolor=olive]{NT: #1}}
\newcommand{\simonl}[1]{\todo[inline, linecolor=red,backgroundcolor=purple!25,bordercolor=purple!75]{SML: #1}}
%%\newcommand{\reviewer1}[1]{\textcolor{orange}{#1}}
%\newcommand{\re1}[1]{\todo[inline,linecolor=black,backgroundcolor=orange!30,bordercolor=red]{R1: #1}}


%math formula overline 
%\newcommand*{\ovC}[1]{\overline{\mbox{#1\strut}}}
%\newcommand*{\ovCC}[2]{\overline{\mbox{#1 $\rightarrow$ #2 \strut}}}

%text overline (good for comments)
\newcommand*{\ovC}[1]{\overline{#1\strut}}
\newcommand*{\ovCC}[2]{\overline{#1 \rightarrow #2 \strut}}

%text color commands
%\red, \green, and \blue are defined with colors for the proofread mode (later inside the setup), however, their default is empty to have no color in other modes
% \newcommand{\red}[{}
% \newcommand{\green}{}
% \newcommand{\blue}{}
\newcommand{\red}[1]{#1}
\newcommand{\green}[1]{#1}
\newcommand{\blue}[1]{#1}
\newcommand{\blu}[1]{\color{black}#1\color{black}{}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Conditional Packages & Commands: 	[by Nima Taherinejad (c)]  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Document Modes: 					[by Nima Taherinejad (c)]  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%default
\newcounter{documentmode}
\setcounter{documentmode}{\mode}
\includecomment{conf}  	%\begin{conf} \end{conf}
%end default
%if case
\newcommand{\setdocmode}{%
  \ifcase\number\value{documentmode}
  	%Proofread Mode (e.g. comment and text color changes)
  	% SML 26.4.2020:
  	% \textcolor is not a "\long\def", so by default you can't use textcolor
  	% for coloring multiple paragraphs or longer sections across environments
  	% (align, tabular etc....)
  	% From xcolor.dtx:
  	%   \def\textcolor#1#{\@textcolor{#1}}
    %   \def\@textcolor#1#2#3{\protect\leavevmode{\color#1{#2}#3}}
    %------------------------------------
    % However, \renewcommand per default defines \long\def commands. So by using
    % \textcolor for \red etc., this property is discarded.
    % Hence I will change the color definitions for now, so I can use them for
    % tables and aligns, too.
% 	\renewcommand{\red}{\textcolor{red}}
% 	\renewcommand{\green}{\textcolor{olive}}
% 	\renewcommand{\blue}{\textcolor{blue}}
    % I am aware that my definition is by no means ideal. But at least its
    % \long so it is much more versatile. And, for the sake of consistency, I
    % will use \renewcommand instead of \def, as you did.
    \renewcommand{\red}[1]{\color{red}##1\color{black}{}}
    \renewcommand{\blue}[1]{\color{blue}##1\color{black}{}}
    \renewcommand{\green}[1]{\color{olive}##1\color{black}{}}
  \or
  	%Draft Mode	
    \usepackage{draftwatermark}
	\SetWatermarkScale{1.35}
	\SetWatermarkAngle{56}
	\SetWatermarkLightness{0.9}
	\SetWatermarkHorCenter{0.9\textwidth}
	\SetWatermarkVerCenter{0.7\textheight}
  \or
  	%Confidential Mode
	\usepackage{draftwatermark}
	\SetWatermarkText{CONFIDENTIAL}
	\SetWatermarkScale{0.67}
	\SetWatermarkAngle{56}
	\SetWatermarkLightness{0.9}
	\SetWatermarkHorCenter{0.6\textwidth}
	\SetWatermarkVerCenter{0.6\textheight}
  \else
    %Final Mode
    \excludecomment{conf}
  \fi
}

\if\mode0
\usepackage[prependcaption, textsize=footnotesize]{todonotes}
\else
\usepackage[disable, prependcaption, textsize=footnotesize]{todonotes}
\renewcommand{\hl}[1]{#1}
\fi

\setdocmode



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Redaction Modes:					[by Nima Taherinejad (c)]  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%default
\newcounter{redmode}
\setcounter{redmode}{\redactionmode}
\includecomment{2Detailed}			%\begin{2Detailed} \end{2Detailed}: 1st level redaction
\includecomment{Uncritical}			%\begin{Uncritical} \end{Uncritical}: 2nd level redaction
\includecomment{2SaveSpace}			%\begin{2SaveSpace} \end{2SaveSpace}: 3rd level redaction
\includecomment{IfMustDelete}			%\begin{IfMustDelete} \end{IfMustDelete}: 3rd level redaction
%end default
\newcommand{\redact}{%
  \ifcase\number\value{redmode}
    \includecomment{2Detailed}
    \includecomment{Uncritical}
    \includecomment{2SaveSpace}
    \includecomment{IfMustDelete}
  \or
    \excludecomment{2Detailed}
    \includecomment{Uncritical}
    \includecomment{2SaveSpace}
    \includecomment{IfMustDelete}
  \or
    \excludecomment{2Detailed}
    \excludecomment{Uncritical}
    \includecomment{2SaveSpace}
    \includecomment{IfMustDelete}
  \or
    \excludecomment{2Detailed}
    \excludecomment{Uncritical}
    \excludecomment{2SaveSpace}
    \includecomment{IfMustDelete}
  \or
    \excludecomment{2Detailed}
    \excludecomment{Uncritical}
    \excludecomment{2SaveSpace}
    \excludecomment{IfMustDelete}
  \fi
}
\redact



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Alternative Text Modes:			[by Nima Taherinejad (c)]  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%default
\newcounter{alttxtmode}
\setcounter{alttxtmode}{\alttextmode}
\includecomment{TextA}			%\begin{TextA} \end{TextA}: Alternative Text A
\includecomment{TextB}			%\begin{TextB} \end{TextB}: Alternative Text B
\newcommand{\alttext}{%
  \ifcase\number\value{alttxtmode}
    \includecomment{TextA}
    \includecomment{TextB}
  \or
    \excludecomment{TextA}
    \includecomment{TextB}
  \or
    \includecomment{TextA}
    \excludecomment{TextB}
  \or
    \excludecomment{TextA}
    \excludecomment{TextB}
  \fi
}
\alttext


